Structural Language Models of Code

We address the problem of any-code completion - generating a missing piece of source code in a given program without any restriction on the vocabulary or structure. We introduce a new approach to any-code completion that leverages the strict syntax of programming languages to model a code snippet as a tree - structural language modeling (SLM). SLM estimates the probability of the program's abstract syntax tree (AST) by decomposing it into a product of conditional probabilities over its nodes. We present a neural model that computes these conditional probabilities by considering all AST paths leading to a target node. Unlike previous techniques that have severely restricted the kinds of expressions that can be generated in this task, our approach can generate arbitrary code in any programming language. Our model significantly outperforms both seq2seq and a variety of structured approaches in generating Java and C# code. Our code, data, and trained models are available at http://github.com/tech-srl/slm-code-generation/ . An online demo is available at http://AnyCodeGen.org .

==> 00-abstract.tex <==
\begin{abstract}
Structured conditioned generation of programs requires reasoning about an infinite number of possible tree structures, assigning the right symbols, as well as fitting these to a given context. 
Prior approaches 
%which addressed similar tasks
were limited to domain-specific languages or to narrow spaces of generated programs. %or to very homogeneous datasets.
%State of the art models for source code generation take the sequence-to-sequence (seq2seq) approach common in machine translation, casting the given context and the target output as separate token sequences.
%We introduce a novel approach
In the general, open-vocabulary, open-structure, settings of this task, the current state-of-the-art is the sequence-to-sequence (seq2seq) approach common in machine translation.
We introduce a new approach that leverages the strict syntax of programs to model the entire code as a single tree: structural language modeling (SLM).
%We introduce a new approach that leverages the strict syntax of programs to model both parts of the code, context and target, as a single tree: tree language modeling (SLM). \omer{I'm not so happy with this sentence, it's a bit bulky.} \eran{I am not loving the SLM terminology, what was wrong with structured?} 
%A tree language model estimates the probability of a program's \omer{code? we're looking at methods after all, not complete programs} abstract syntax tree (AST) by decomposing it into a product of conditional probabilities over its nodes.
A structural language model estimates the probability of the program's abstract syntax tree (AST) by decomposing it into a product of conditional probabilities over its nodes.
We also present a neural model for computing these conditional probabilities using all AST paths leading up to a target node.
Our model significantly outperforms both seq2seq and a variety of existing structured approaches in Java and C\#.
We make our code, datasets, and trained models publicly available.

% Structured conditioned generation of programs requires reasoning about an infinite number of possible tree structures, assigning the right symbols, as well as fitting these to a given context. 
% Prior approaches which addressed similar tasks  were limited to domain-specific languages or to narrow spaces of generated programs. %or to very homogeneous datasets.
% We present a novel open-vocabulary, open-structure, and general-purpose structural language model for generating \emph{any} code node-by-node.
% %, conditioned on the surrounding code context. 
% %Our model encodes the available symbols, actions and their syntactic relation to the target prediction; uses self-attention to propagate information between context items; and generates the target syntax tree node-by-node.
% We demonstrate the effectiveness of our approach for generating code in two programming languages, outperforming a variety of strong state-of-the-art baselines. We make our code, datasets, and trained models publicly available.
\end{abstract}



==> 01-intro.tex <==
\section{Introduction}
\label{Intro}

\omer{I think we need to completely rewrite the intro to reflect the narrative in the abstract.

Par 1: Task of any code gen, contrast with prior work on restricted

Par 2: In this task, sota is seq2seq+copy (forward ref to results?)
however, (1) code is structured, (2) the input and output are parts of a common entity, not 2 different modalities.
our solution: LM on AST

Par 3:
* describe the decomposition (DFS)
* paths as inputs
* implementation: neural model with copy

Par 4:
* results
*** don't forget: prior art doesn't beat seq2seq+copy
* ablations
}

Learning to generate programs is one of the oldest problems in machine learning \cite{waldinger1969prow} and has been considered by some as the ``holy grail of computer science'' \cite{pnueli1989synthesis, gulwani2017program}. In its general form, it requires reasoning about some given context along with the semantic and syntactic information it provides, as well as generating valid and likely code.
Since this problem is extremely hard, most prior approaches chose to limit the problem in various aspects: program synthesis approaches \cite{manna1971toward} have been tailored to domain-specific languages (DSLs) \cite{gulwani2011automating, polozov2015flashmeta} that
%- while this works well for some tasks, DSLs 
%are (literally) domain-specific and 
do not generalize to other domains and tasks; semantic parsing approaches usually address highly templated datasets \cite{ling2016latent, shin2019idioms} or templated languages like SQL \cite{yu2018spider, dong2018coarse}; other recent approaches generate code in general languages like Java and C\#, but heavily restrict the type of code they can generate \cite{murali2018bayou, brockschmidt2018generative}. %; and other works required additional  input \cite{iyer2018mapping, chen2018tree, kulal2019spoc}. 
In this paper, we consider the general problem of filling in code within a partial program in general-purpose programming languages.

In the general-language, open-vocabulary, scenario we address, the current state-of-the-art is the sequence-to-sequence (seq2seq) approach with a copy mechanism (as we show in \Cref{sec:results}). However, 
%while sometimes performing surprisingly well (as we show in \Cref{evaluation}) 
this approach does not consider the structure of the programming language and thus wastes capacity by implicitly re-learning the (known) grammar of the language. Further, we recognize that, in this task, the input and the target code are of the \emph{same modality}: code$\rightarrow$code, rather than NL$\rightarrow$code \cite{yin2017, rabinovich2017} or input/output examples-to-code \cite{parisotto2016neuro, devlin2017robustfill}.
These observations motivate us to address this task with a \emph{structural language model} (SLM)
, which is fundamentally different than encoder-decoder models such as \citet{brockschmidt2018generative} and \citet{murali2018bayou}. 

We present a novel approach for \emph{any} code generation given the surrounding code context. We employ Abstract Syntax Tree (AST) paths \cite{alon2019code2seq} that have been shown to capture semantically meaningful representations for encoding programs. Nonetheless, while \citet{alon2019code2seq} use paths to encode pre-existing programs, we \emph{generate code} and thus learn to \emph{extend} partial paths with the next node. Our model generates the target syntax tree node-by-node by predicting the next AST node of multiple paths, conditioned on the syntactic relation to all symbols and actions in the context. 


%. For example, 
%\citet{yin2017} proved the application of their approach only to highly templated datasets; 
%\citet{murali2018bayou} require API-heavy data, and thus cannot generate general or logical-only programs; \citet{brockschmidt2018generative} generate only expressions of primitive types (boolean, arithmetic, or string) or arrays of these, excluding calls to user-defined functions.


%To that end, we introduce the Any Expression Generation (\aeg) of filling in an expression of \emph{any type}, \emph{any structure}, and containing \emph{any code},
%within an existing partial program.




%This is different than most previous work, since these usually generate code as a sequence of \emph{production rules}. 
%\omer{It is hinted, but not entirely clear at this point, that we are doing code completion. I think that, although the first couple of paragraphs are very well written, they are speaking very broadly about code generation, and we might need to replace them with ones that position this paper as a code completion paper. It will scope the paper more tightly, and thus prevent reviewer \#2 from saying that we're over-claiming our contributions.} \uri{I totally agree - this is code completion. It's just that the term "code completion" is problematic - it hints to something more software-engineeric, and that the completion might be a single token (rather than a complete expression). Not using "completion" is actually a smart rhetoric move that Marc Brockschmidt from MSR did in his ICLR'19 paper.} \omer{We can definitely avoid the term code completion, as long as we clearly scope and define the task in the first paragraph. For example: "We focus on generating any code (expressions/statements/functions/whatever) given surrounding code as input."} \uri{It is written in the beginning of the 3rd paragraph, because it doesn't fit in the first two... Do you think we should move it to the first paragraph? it doesn't fit the story. Para1 is about how code generation (in general) is important; Para2 is about how all previous approaches are limited (regardless of their exact input type)} \eran{I think we need a new term that is not ``completion'' maybe ``local generation'' or ``local synthesis'' or something like that. Also, ``code completion'' is not entirely appropriate if we also condition on code after the ``hole''.}

%We demonstrate our approach in a novel architecture that includes Transformer layers \cite{vaswani2017attention} on top of LSTM states. 
%We use LSTMs to encode partial AST paths, and self-attention to capture the interaction between all partial paths.
%We assign symbols by combining a small \emph{sub}token vocabulary with a syntactic copy mechanism, and can thus generate open vocabulary and out-of-vocabulary tokens. 
%\omer{These last three sentences might be TMI for an intro.} \uri{kept only the first one, to counter the usual argument: "AST paths are not novel, LSTMs are not novel $\implies$ your work is not novel"}
We show that our approach generalizes most previous work under a joint framework, without the ``highly complex form of feature engineering'' \cite{brockschmidt2019graph} involved in mapping programs to, for example, graphs.
%\uri{nice move, huh? He actually said that graphs are feature engineering! I'm proud of myself} \omer{+1 :)}. 
We demonstrate the effectiveness of our approach in generating general-purpose unlimited expressions in two languages and comparing to a range of strong baselines \cite{brockschmidt2019graph,yin2017,iyer2018mapping,alon2019code2seq}, as well as state-of-the-art NMT models \cite{luong15, vaswani2017attention, aharoni2017towards}. %\omer{I would elaborate on the results, and consider quoting actual numbers in the introduction.} \uri{done}
Compared to the strongest NMT baseline, our model achieves over $1.1\%$ and $1.6\%$ absolute gains on \emph{accuracy@1} and \emph{accuracy@5} respectively.
Compared to the model of \citet{brockschmidt2018generative} in their restricted settings, we achieve absolute gains of over $22\%$ and $18\%$. 
To examine the importance of different components in our approach, we conduct a thorough ablation study;
specifically, we show the great advantage of a joint structural language model over encoder-decoder models that model the source and the target as different modalities.
%We make our code, trained models and a new Any Expression Generation dataset publicly available.
%Finally, our model relies purely on the syntax of the generated programming language, thus not assuming any properties or knowledge of the language or the data.


==> 02-background.tex <==
\section{Representing Code as a Tree}
\label{sec:background}

A program $\mathcal{P}$ is a sequence of tokens in a certain language, which is unambiguously equivalent to an abstract syntax tree (AST) $\mathcal{A_P}$. 
The leaves of the AST (terminals) have an additional associated user-defined value $v \in \mathcal{V}$.  
The non-leaf nodes (nonterminals) can have a varying number of children nodes.
Each nonterminal represents a structural element in the language (e.g. conditions, loops, variable declarations) from a closed set $\mathcal{T}$.

In this work, we augment the AST $\mathcal{A_P}$ by adding each terminal node's value $v$ as a subtree $T_v$ under each terminal node.
Specifically, we decompose $v$ into subtokens according to camel notation, and define $T_v$ as a sequence of terminal nodes with subtoken values. For example, if $v=\scode{toLowerCase}$, then $T_v = \scode{to} \rightarrow \texttt{lower} \rightarrow \texttt{case}$.
% \begin{align*}
% v=\texttt{equalsIgnoreCase} & & T_v = \texttt{equals} \rightarrow \texttt{ignore} \rightarrow \texttt{case}
% \end{align*}
% \begin{align*}
% v=\texttt{equalsIgnoreCase} & & T_v = \texttt{equals} \rightarrow \texttt{ignore} \rightarrow \texttt{case} \rightarrow \texttt{EOS}_{tok}
% \end{align*}
% The $\texttt{EOS}_{tok}$ subtoken is a special marker that denotes the end of the token.
% We use a similar marker $\texttt{EOS}_{node}$ to denote the number of children in 

==> 02-task.tex <==
\section{Task: Any-Code Generation}\label{sec:background}
\input{task_example_fig_horizontal}
\omer{I'm thinking of merging this whole section into the intro. It basically has three important sentences: 1) The task is filling missing code. 2) The missing code is assumed to be a valid sub-AST. 3) This is a much more general task than Brockstein et al. }
\eran{yes, I agree, this should be part of the intro.}

We introduce the Any-Code Generation (\aeg) task of filling in \emph{any code}, of \emph{any type}, and \emph{any structure}, within an existing partial program.
% \paragraph{Notation}
% A program $\mathcal{P}$ in a certain programming language $\mathcal{L}$ is a sequence of tokens $k_1,...,k_{\left| \mathcal{P}\right|}$, which is unambiguously equivalent to an Abstract Syntax Tree (AST) $\mathcal{A_P}$. 
% An AST is a tree in which every node belongs to a predefined set $\mathcal{N}$; the leaves of the tree, also called \emph{terminals}, have an additional associated user-defined value.

\para{Notation}
A program $\mathcal{P}$ in a certain programming language $\mathcal{L}$ is a sequence of tokens $k_1,...,k_{\left| \mathcal{P}\right|}$ which is unambiguously equivalent to an Abstract Syntax Tree (AST) $\mathcal{A_P}$. An AST is a tree in which every node belongs to a predefined set $\mathcal{N}$; the leaves of the tree, also called \emph{terminals}, have an additional associated user-defined value $v\in \mathcal{V}$.  The non-leaf nodes, also called \emph{nonterminals}, can have a varying number of children nodes, and they represent the set of structures in the language such as conditions, loops, and variable declarations. 
%We consider the problem of learning the conditional probability $Pr\left(p|\mathcal{P^{-}}\right)$, where $p$ is a piece of the program $k_{i+1},...,k_{i+\left|p\right|}$ \uri{$p$ is defined here} which is equivalent to the sub-AST $a_{\mathcal{P}}$; and $\mathcal{P^{-}}$ is the program where $p$ was \emph{removed}: $k_1,...,k_i,k_{i+\left|p\right|+1},...,k_{\left| \mathcal{P}\right|}$, which is equivalent to the partial AST $\mathcal{A^{-}_P}$. Learning the probability $Pr\left(p|\mathcal{P^{-}}\right)$ is thus equivalent to learning $Pr\left(a_{\mathcal{P}}|\mathcal{A^{-}_P}\right)$. 

\para{Task Definition}
Given a program $\mathcal{P}$ and some part of the program $p=k_{i+1},...,k_{i+\left|p\right|}$, we consider the problem of predicting $p$ from the rest of the program $\mathcal{P^{-}} = \mathcal{P} \setminus p=k_1,...,k_i,k_{i+\left|p\right|+1},...,k_{\left| \mathcal{P}\right|}$. %\omer{I moved the conditional probability to the next section, because casting the task as probability estimation is a modeling choice. We also don't evaluate the probabilities directly (e.g. ppl), but evaluate the actual productions (e.g. BLEU).}
The only restriction we place is that $p$ must have a valid sub-AST, denoted as $\mathcal{A}_{p}$. 

%An AST is a tree in which every node belongs to a predefined set $\mathcal{N}$; the leaves of the tree, also called \emph{terminals}, have an additional associated user-defined value.
%\omer{maybe add a sentence about what this means for the sequence of tokens? e.g. do they have to be contiguous? do they have to be a valid expression?}
%\omer{add citations about others who modeled the code as an AST? (e.g. "syntactic approaches")}

\para{Example}
\Cref{fig:task_example} shows two \aeg{} examples from our test sets in Java (\Cref{fig:task_example_a}) and C\# (\Cref{fig:task_example_b}), along with the expressions generated by our models. These generated expressions can contain user-defined and library types, e.g., \scode{FileStatus} and and \scode{StringBuilder}, and various structures such as array indexing, method call (\Cref{fig:task_example_a}), and overloaded operator call (\Cref{fig:task_example_b}). Our model generates these expressions correctly, by combining in-vocabulary tokens with tokens that are copied from the context. More examples can be found in Appendices C-D.%\Cref{appendix:java_examples} 
%(Java)
% and \Cref{appendix:csharp_examples}. % (C\#).

% We consider the problem of learning the conditional probability $Pr\left(p|\mathcal{P^{-}}\right)$, where $p$ is a piece of the program $k_{i+1},...,k_{i+\left|p\right|}$, which is equivalent to the sub-AST $a_{\mathcal{P}}$, and $\mathcal{P^{-}}$ is the program where $p$ was \emph{removed}: $k_1,...,k_i,k_{i+\left|p\right|+1},...,k_{\left| \mathcal{P}\right|}$, which is equivalent to the partial AST $\mathcal{A^{-}_P}$. Learning the probability $Pr\left(p|\mathcal{P^{-}}\right)$ is thus equivalent to learning 
% $Pr\left(a_{\mathcal{P}}|\mathcal{A^{-}_P}\right)$. 

% We introduce the \textsf{AnyExprGen} task of filling in an expression of \emph{any type}, \emph{any structure} and containing \emph{any code},
% within an existing partial code of a general-purpose programming language. \uri{show example}. This task requires generating a likely tree structure, copy symbols from the partial context program, as well as generating new unseen tokens that may contain in-vocabulary with in-context subtokens.

%\paragraph{Prior Work}
This task generalizes the Expression Generation (ExprGen) of \citet{brockschmidt2018generative}, 
in which the target code contains only primitive types (boolean, arithmetic, or string) or arrays of these,
%is taken from a limited set of expression types, 
and does not include calls to user-defined functions. 
%generate only expressions of primitive types (boolean, arithmetic, or string) or arrays of these, excluding calls to user-defined functions.
In the rest of the paper, we will refer to these restricted settings as Restricted Code Generation (RestrictGen).

\omer{move description of ASTs here, including the breaking down of subtokens to linear subgraphs} \uri{Tried, it didn't feel appropriate,  moved it back to Sec 3}

\omer{Define the tree structure (e.g. that the subwords of an identifier are also nodes, etc). Perhaps even show the EOS tokens.} \uri{Tried, it didn't feel appropriate,  moved it back to Sec 3}


==> analysis.tex <==
\section{Ablation Study}
\label{sec:ablation}
To understand the important of the various components and design decisions in our model, we conducted an extensive ablation study. The following experiments were performed on the Java dataset and \textsf{AnyExprGen} task. We examined several alternative models:
\begin{enumerate}
\item \emph{No copy} - does not use a copying mechanism, but uses a much larger vocabulary instead ($10,000$ subtokens instead of $1000$).
\item \emph{Paths$\rightarrow$seq} - separates the model to an encoder and a decoder, where the decoder generates the target expression as a sequence of subtokens (including a copy mechanism).
\item \emph{Seq$\rightarrow$Paths} - separates the model to an encoder and a decoder (including a copy mechanism), where the encoder encodes the context as a sequence of subtokens using a BiLSTM, and the decoder uses root paths and only paths starting in already-expanded leaves ($\mathrm{leaves\left(a_{\mathcal{P}_{<t}}\right)}$). 
\item \emph{Tree-idioms} - follows the spirit of \citet{shin2019idioms} and collects the $50$ mostly occurring tree-idioms in the training data; these form more than $75\%$ of the training target examples. The model is then trained to emit the entire idiom in a single step, and then fill the missing subtokens, while still having the ability to generate the target tree node-by-node as usual. Differently from \citet{shin2019idioms}, in this experiment idioms contained only AST nodes (e.g., \fbox{\scode{NAME > INT}}), without subtoken value assignments (i.e., the actual values of \scode{NAME} and \scode{INT}), and are collected by simply taking the most frequent trees.
\item \emph{No root path} - does not use of the path from the root to the expanded node (marked as $\mathcal{R}$ in \Cref{fig:greater}). Instead, $g$ uses max-pooling over the Transformer-encoded vectors $z_1,...,z_{|\mathcal{T}_{\upsilon}|}$.
\item \emph{No Transformer layers} - \uri{I will remove this, we should avoid focusing on the exact architecture} uses exactly the same architecture as SLM, without the Transformer encoder layers. That is, $z_1,...,z_{|\mathcal{T}_{\upsilon}|}$ are the encoded partial paths $\mathbf{h}_1,...,\mathbf{h}_{|\mathcal{T}_{\upsilon}|}$.
\end{enumerate}

\Cref{tab:csharp-unlimited-results} shows the results of these alternatives. 
As shown, \emph{not using a copying mechanism} results in a degradation of about $46\%$. Programs use symbols and identifiers repetitively, thus the ability to copy symbols from the context is crucial. For this reason, we included a copying mechanism in all NMT baselines in \Cref{evaluation}. 
\emph{Paths$\rightarrow$seq} and \emph{Seq$\rightarrow$Paths} show the great benefit of using a \emph{structural language model}. This shows that the \textsf{AnyExprGen} task should be addressed as a language modeling problem, since separating the model to encoders and decoders of different types significantly degrades the generalization ability of the model.
Using \emph {Tree-idioms} degrades the results by about $\%7$-$\%8$. We hypothesize that the exact settings and mining process used in \citet{shin2019idioms} are crucial; alternatively, idioms might be helpful in more templated datasets like Hearthstone \cite{ling2016latent} and languages like SQL
% (Spider dataset \cite{yu2018spider}, 
which were all used by \citet{shin2019idioms}.
%\emph{Paths$\rightarrow$seq} performs slightly better than \emph{Seq$\rightarrow$Paths}; we hypothesize that 
\emph{No root path} degrades \emph{acc@1} and \emph{acc@5} by $19\%$-$26\%$. This shows the contribution of explicitly using the relative position in the program, expressed as the path from the root, even though the root path is necessarily included as a sub-path of other paths in the set $\mathcal{T}_{\parent}$.
%\emph{No Transformer layers} shows that using the Transformer encoder layers provides more expressivity because they allow the paths to interact with each other before predicting the next node. Even without Transformer layers, the model achieved slightly higher results than all baselines in \Cref{tab:java-results}.

\begin{table}[t]
\scriptsize
\hspace{-2mm}
\begin{minipage}{0.5\textwidth}
% C# AnyExprGen table starts here
\caption{Our model outperforms graph-based baselines in unlimited code generation (\textsf{AnyExprGen}) in C\#. $\dagger$Baselines implemented by \citet{brockschmidt2018generative} and re-trained by us.}
\label{tab:csharp-unlimited-results}
\begin{tabular}{lrrrr}
\toprule
%\multirow{2}{*}{Model}              & \multicolumn{4}{c}{Unlimited Expressions (\textsf{AnyExprGen}) }    \\
%\cmidrule{2-5} 
Model                & Acc@1     & Acc@5     & Tree@1   & Tree@5  \\
\midrule
$G\!N\!N\!\!\rightarrow\!\!\mathcal{N\!\!AG}^{\dagger}$  & 3.49 & 5.07 &6.45 &9.03  \\
$seq$$\rightarrow$$seq^{\dagger}$ & 2.67 & 4.05 & 27.17 & 35.08 \\
$seq$$\rightarrow$$graph^{\dagger}$  & 1.48 & 2.26 & 3.35 & 4.66 \\
$graph$$\rightarrow$$seq^{\dagger}$  & 7.53 & 9.63 & 33.95 & 41.39\\
\midrule %[\heavyrulewidth]
SLM (this work) & \textbf{14.86}  & \textbf{24.38}  & \textbf{61.62}  & \textbf{76.61}  \\
\bottomrule
\end{tabular}
\end{minipage}
\hspace{2mm}
% ABLATION TABLE STARTS HERE
\begin{minipage}{0.5\textwidth}
\caption{Variations of our SLM model compared to the original model.}
\label{tab:ablation-results}
% \footnotesize
\centering
\makebox[\linewidth]{
\begin{tabular}{lrrrr}
\toprule
%\multirow{2}{*}{Model}              & \multicolumn{2}{c}{Exact Match}    & \multicolumn{2}{c}{Tree-only}    &    \\
%\cmidrule{2-3} \cmidrule{4-5} 
Ablation          & Acc@1     & Acc@5     & Tree@1   & Tree@5  \\
\midrule
No copy & 9.55  & 13.47 & 29.91 & 44.20\\
Paths$\rightarrow$seq & 12.95 & 18.52  & 33.44 & 43.43 \\
Seq$\rightarrow$Paths & 10.99 & 15.85 & 28.02 & 43.05 \\
Tree idioms & 16.59 & 23.04 & 36.89 & 51.10 \\
No root path & 14.43 & 18.48 & 28.20 & 35.65 \\
%No Transformer layers\uri{remove} & 17.59 & 24.36 & 36.73 & 53.35\\
\midrule
SLM (original model) &  17.81 & 25.03 & 37.72 & 53.88 \\
\bottomrule
\end{tabular}
}
\end{minipage}
\end{table} 

==> csharp_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table}[t]

%}
\end{table} 

==> efficient_subfigure.tex <==
\includegraphics[height=5cm,keepaspectratio]{figures/efficient_fig.pdf}
\end{center}
\caption{Efficient computation: partial paths for different time steps share the same prefix, allowing a shared computation. In this example, the prefix is the shared path from the leaf (not shown) to \scode{Greater}, and is much longer than either of the suffixes.}
\label{fig:efficient}

==> eos_and_efficient_figures.tex <==
%\begin{wrapfigure}{R}{0.20\textwidth}
\begin{figure*}[t]
\centering
\begin{minipage}{0.30\textwidth}
%\begin{subfigure}[t]{1.0\textwidth}
\begin{center}
% \vspace{-5mm}
\input{eos_subfigure.tex}
%\end{subfigure}
%\end{wrapfigure}
\end{minipage}
\hspace{6mm}
\begin{minipage}{0.62\textwidth}
%\begin{wrapfigure}{R}{0.3\textwidth}
%\begin{subfigure}[t]{1.0\textwidth}
\begin{center}
%\vspace{-5mm}
\input{efficient_subfigure.tex}
%\end{wrapfigure}
%\end{subfigure}
\end{minipage}
\end{figure*}

==> evaluation.tex <==
%\newcommand{\gnntonag}{$G\!N\!N\!\!\!\!\rightarrow\!\!\mathcal{N\!AG}$}
\newcommand{\gnntonag}{$G\!N\!N$$\rightarrow$$\mathcal{N\!AG}$}

\section{Experiments}\label{evaluation}

\omer{Consider the following layout: 5.1 Benchmarks, 5.2 Baselines, 5.3 Implementation (which will include hyperparameters and miscellaneous details that are important for replication), 5.4 Results.} \uri{done} \omer{Depending on what we do for ablations, it might also make sense to move the results into a separate section of their own, making this section just "Experimental Setup".}

\subsection{Benchmarks}
\paragraph{Java Dataset}
We use the Java-small dataset of \citet{alon2019code2seq} which is a re-split of the dataset of \citet{conv16}, but splits to training-validation-test across projects. This dataset was found to contain the least code duplication by \citet{allamanis2018adverse}. We used this dataset for the \textsf{AnyExprGen} task: as target examples we took all expressions (\scode{node instanceof Expression}) that are larger than a single node. We removed methods which contained the word ``test'' in their body or file name, and methods larger than $20$ lines, because these were often auto-generated code, large configuration files, or other unusual methods. To make the task even harder, we removed examples in which the target subtree appeared as-is in the context (i.e., the target expression is \fbox{\scode{x > 1}} and \fbox{\scode{x > 1}} also appears somewhere else in the context). These resulted in $1.3M$ training examples.

\paragraph{C\# Dataset}
Since the dataset of \citet{brockschmidt2018generative} is not publicly available, we consulted with the authors and used the dataset of \citet{allamanis2018learning} to ensure a qualitative dataset which is low in code duplication. We used the same raw dataset for \textsf{ExprGen} and \textsf{AnyExprGen}, extracting different subsets of examples. For the \textsf{ExprGen} task, which is limited to only primitive types and excludes user-defined functions, we extracted the exact same types of limited expressions using the code of \citet{brockschmidt2019graph}. 
%this resulted in $16.3K$ training examples. 
For our new \textsf{AnyExprGen} task, we used the same raw dataset to extract any expression larger than a single node, with additional cleaning as in the Java dataset.
%this resulted in $336K$ training examples.

Statistics of all datasets are provided in \Cref{statistics}

\paragraph{Metrics}
%As we consider our model as a conditional structural language model, we measure the perplexity of the model exactly as measured by \citet{brockschmidt2018generative}. 
We perform beam search with width of $5$, follow \citet{brockschmidt2018generative} and report the exact match accuracy at $1$ and at $5$. Additionally, we introduce a new \emph{tree@k} metric, which is similar to ``exact match'' except that it ignores leaf values; instead, \emph{tree@k} counts a prediction as correct if the entire tree structure, ignoring leaf values, is identical to the tree of the ground truth. 
For example, the expressions \fbox{\scode{x > 1}} and \fbox{\scode{y > 2}} would \emph{not} count as identical in ``exact match'', but \emph{would} count as ``tree-only identical'' because both express that an \emph{identifier} is \emph{greater} than an \emph{integer}.
The \emph{tree@k} metric is interesting because succeeding in \emph{tree@k} hints that there is room to overall improve the model by improving token value assignment. \uri{We don't measure BLEU over tokens like Iyer'18 and Shin'19, because I don't think it's very useful... Do we want to say something about this? Or is it arrogant?}

\subsection{Baselines}
%\paragraph{Baselines}
\omer{This part needs to be promoted into a subsection, and provide more detail about each method. A lot of the stuff that's currently in related work should move here.} \uri{Made it a subsection, not sure which part of the related work should move here?}
We compare our model to original implementations where available and adaptations of NMT architectures. We put significant effort to perform a fair comparison, including adding a copying mechanism to the NMT baselines and \emph{sub}tokenization. We adapted strong baselines from the literature to our task, even if they were designed to different tasks such as NL$\rightarrow$code and code$\rightarrow$NL. We re-trained all the following baselines on the same datasets as our model.

\paragraph{Java baselines}
In Java, we used the original implementation of \citet{iyer2018mapping}, and also their \emph{Seq2Prod} baseline which is a re-implementation of \citet{yin2017}; both are designed for NL$\rightarrow$code tasks, in which we feed the (sub)tokenized code context as input. We compare to \emph{code2seq} \cite{alon2019code2seq}, which is the state-of-the-art code$\rightarrow$NL model, and train it to generate the target code as a sequence of subtokens. We also compare to NMT baselines, in which we \emph{sub}tokenize the given code snippet, replace the target in the source with a special \scode{PRED} symbol, and train the network to predict the target as a sequence of subtokens: \emph{Transformer} \cite{vaswani2017attention}+copy uses the implementation of OpenNMT \cite{2017opennmt} with the default hyperparameters and a copy mechanism \cite{gu2016incorporating}; \emph{BiLSTM$\rightarrow$LSTM+copy} is a 2-layer bidirectional LSTM with $512$ units encoder-decoder and attention \cite{luong15}; \emph{Seq2tree+copy} follows \citet{aharoni2017towards} and learns to generate the linearized, subtokenized target AST, with the same architecture as \emph{BiLSTM$\rightarrow$LSTM+copy}.

\paragraph{C\# baselines}
For the \textsf{ExprGen} task in C\#, \gnntonag{} is the original implementation of \citet{brockschmidt2018generative}, who implemented additional baselines: $seq$$\rightarrow$$seq$, $seq$$\rightarrow$$graph$, and $graph$$\rightarrow$$seq$ which follows \citet{fernandes2018structured}. Similarly to Java, we compared to \emph{code2seq}, \emph{Transformer+copy}, \emph{BiLSTM$\rightarrow$LSTM+copy} and \emph{Seq2tree+copy}. 
In the \textsf{AnyExprGen} task in C\#, we compared our model to the graph-based models and baselines of \citet{brockschmidt2018generative}.

\subsection{Implementation}
We use embeddings of size $512$, $L=2$ layers of LSTMs with $256$ units, and $N_T=3$ Transformer layers with $N_H=4$ attention heads. We kept a subtoken vocabulary of size $1000$ to encourage the model to learn to copy; larger vocabularies did not show an improvement. This resulted in a very lightweight model of only $13M$ trainable parameters.

\paragraph{Training} We train the model end-to-end using the cross entropy objective and the Adam optimizer \cite{kingma2014adam}, an initial learning rate of $5\cdot10^{-4}$ decayed by a factor of $0.95$ every $20,000$ steps. 
The cross entropy loss derived from predicting AST nodes and this of predicting subtokens are averaged according to their numbers in each batch with equal weights.
We bucket examples into the same batch based on the number of target predictions
%in the target subtree 
(nodes + subtokens + EOS symbols), and vary the batch size accordingly. 
We train the model to copy full tokens if available, and otherwise construct tokens by mixing in-vocabulary subtokens with copied subtokens.
We apply dropout of $0.25$ in the self-attention and the Transformer feedforward layers, and a recurrent dropout of $0.5$ on the LSTMs. 

\subsection{Results}	

\input{java_results.tex}
\input{csharp_results.tex}

\paragraph{Performance - Java} 
\Cref{tab:java-results} summarizes the results for the \textsf{AnyExprGen} task in Java. Our model achieves more than $5\%$ and $8\%$ relative gains on \emph{acc@1} and \emph{acc@5} respectively over the strongest \emph{BiLSTM$\rightarrow$LSTM+copy} baseline, and over all the other baselines. 
Interestingly, \emph{Seq2tree} achieved higher \emph{tree@k} results than the rest of the baselines, and even $0.42\%$ higher \emph{tree@1} score than our model, while achieving lower results at \emph{acc@1}, \emph{acc@5} and \emph{tree@5}. The most frequent correctly predicted trees by \emph{Seq2tree} were: \fbox{\scode{NAME}.\scode{NAME}()}, \fbox{\scode{NAME}.\scode{NAME}} and \fbox{\scode{NAME}()}.
%\uri{TODO the following sentence. Seq2tree is slightly better at tree@1, where the most common trees are: Cal(Nm(),Nm()), Fld(Nm(),Nm()), StaticCall(Nm())}
%Interestingly, the relative improvement of our model over the best baseline on \emph{Tree@k} is even higher: $29\%$ and $37\%$.% in \emph{Tree@1} and \emph{Tree@5} respectively. 
%This hints that even when both our model and the baselines could not generate the target code exactly, our model was more accurate in predicting the correct tree structure.

\paragraph{Performance - C\#} 
\Cref{tab:csharp-limited-results} shows the results for the \textsf{ExprGen} task in C\#. Our model achieves relative gains of $137\%$ and $58\%$ on \emph{acc@1} and \emph{acc@5} respectively over the state-of-the-art model of \citet{brockschmidt2018generative}, who introduced this task, and over the other baselines. Only 
$graph$$\rightarrow$$seq$ achieves slightly higher 
\emph{tree@5} than our model, $63.75$ compared to our $59.82$, but the exact match accuracy of this baseline is significantly lower. These correctly predicted trees are mostly very simple expressions, where the most frequent correctly predicted trees by $graph$$\rightarrow$$seq$ are \fbox{\scode{NAME * INT}}, \fbox{\scode{NAME[INT]}} and \fbox{\scode{NAME++}}.

\Cref{tab:csharp-unlimited-results} shows the results for the \textsf{AnyExprGen} task in C\#. We note that the graph-decoding models (\gnntonag{} and $seq$$\rightarrow$$graph$) were not designed for this general code generation task, and failed mostly because their implementation could express only about $12\%$ of the target expressions in the test set. This comparison was mostly intended to show the inability of these models to generate general code, as most code in ``the wild'' does not fit into the strict criteria  employed by \citet{brockschmidt2018generative}. %Interestingly, the $graph$$\rightarrow$$seq$ baseline, which \emph{could} express all test examples, achieved the closest results to our model, while our model gained a relative improvement of $4\%$ and $33\%$ on \emph{acc@1} and \emph{acc@5} respectively.


==> expand.tex <==
\begin{figure} 
\centering
\begin{minipage}{0.7\textwidth}
\centering
\begin{algorithm}[H]
\footnotesize
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
%\SetAlgoLined
\SetAlgoNoEnd
\Input{partial AST $\mathcal{A^{-}}$, initial node to expand $a_0$}
\Output{subtree $\tau$}
 $stack\leftarrow$ {emptyStack}();
 {push}($stack$, $a_0$)\;
 $\tau \leftarrow$ {initTree}($a_0$) \;
 \While{stack \normalfont{is not empty}}{
  $parent\leftarrow$ {pop}($stack$)\;
  $\mathcal{S}$ $\leftarrow$ {encodePaths}($\mathcal{A^{-}}$,$\tau$, parent)\;
  \If{parent $\in nonterminals$}{
   $a$ $\leftarrow$ {predictNode}($\mathcal{S}$, $parent$)\;
  }
  \ElseIf{$parent \in terminals$ \normalfont{or} $parent \in subtokens$}{
   $a$ $\leftarrow$ {predictSubtoken}($\mathcal{S}$, $parent$)\;
   }
  \If{a \normalfont{is not} \scode{EOS}}
  {
    $\tau \leftarrow ${insertChild}($\tau$, $parent$, $y$)\;
   {push}($stack$, $a$)\;
  }
 }
 return $\tau$\;
 \caption{Pseudocode for the code generation algorithm.}
 \label{algo:generate}
\end{algorithm}
\end{minipage}
\end{figure}

==> genericmacros.tex <==
%!TEX root=draft.tex

% Generic macros (nothing specific to this paper)

\usepackage{ifthen}
%
\newcommand{\todoi}[1]{{\todo[inline]{#1}}}
\newcommand{\todolow}[1]{}
% \newcommand{\TODO}[1]{ {\color{blue} {\bf #1}} }
\newcommand{\TODO}[1]{ {\color{blue} \bf #1} }
\newcommand{\DONE}[1]{ {\color{gray} \textbf{DONE - } #1} }
\newcommand{\OMIT}[1]{ {\color{gray} \bf #1} }
\newcommand{\AWK}[1]{ {\color{red} \bf #1} }
\newcommand{\TODOFN}[1]{ \footnote{{\bf #1}} }
\newcommand{\COMMENT}[1]{}
\newcommand{\ignore}[1]{}
\newcommand{\ie}{i.e.}
\newcommand{\eg}{e.g.}

%%% references definition
\newcommand{\lemref}[1]{Lemma~\ref{Lm:#1}}
%\newcommand{\figref}[1]{Fig.~\ref{Fi:#1}}
\newcommand{\defref}[1]{Definition~\ref{De:#1}}
\newcommand{\theref}[1]{Theorem~\ref{Th:#1}}
\newcommand{\tabref}[1]{Table~\ref{Ta:#1}}
%\newcommand{\secref}[1]{Section~\ref{Se:#1}}
\newcommand{\secrefs}[2]{Sections~\ref{Se:#1}-\ref{Se:#2}}
\newcommand{\ssecref}[1]{Sec.~\ref{Se:#1}}
\newcommand{\appref}[1]{Appendix~\ref{Se:#1}}
\newcommand{\exref}[1]{Example~\ref{Ex:#1}}
\newcommand{\algref}[1]{Algorithm~\ref{Alg:#1}}
\newcommand{\lnref}[1]{Line~\ref{Ln:#1}}
\newcommand{\slnref}[1]{\ref{Ln:#1}}

\newcommand{\lemlabel}[1]{\label{Lm:#1}}
\newcommand{\figlabel}[1]{\label{Fi:#1}}
\newcommand{\deflabel}[1]{\label{De:#1}}
\newcommand{\thelabel}[1]{\label{Th:#1}}
\newcommand{\tablabel}[1]{\label{Ta:#1}}
\newcommand{\seclabel}[1]{\label{Se:#1}}
\newcommand{\sseclabel}[1]{\label{Se:#1}}
\newcommand{\applabel}[1]{\label{Se:#1}}
\newcommand{\exlabel}[1]{\label{Ex:#1}}
\newcommand{\alglabel}[1]{\label{Alg:#1}}
\newcommand{\lnlabel}[1]{\label{Ln:#1}}

\theoremstyle{definition}
\newtheorem{definition}{Definition}[]

%% TO Allow writing the TR in the same source
\newboolean{TR}
\setboolean{TR}{false}
\ifthenelse{\boolean{TR}}{
\newcommand{\TrSelect}[2]{#1}
\newcommand{\TrOnly}[1]{#1}
\newcommand{\SubOnly}[1]{}
\newcommand{\TrOnlyInFootnote}[1]{#1}
\newcommand{\TrOnlyInTable}[1]{#1}}
{
\newcommand{\TrSelect}[2]{#2}
\newcommand{\TrOnly}[1]{}
\newcommand{\SubOnly}[1]{#1}
\newcommand{\TrOnlyInFootnote}[1]{}
\newcommand{\TrOnlyInTable}[1]{}}

%% General macros
\newcommand{\Set}[1]{\{ \; {#1} \; \}}
\newcommand{\vbar}{\; | \;}
\newcommand{\notIn}{\not\in}
\newcommand{\sizeof}[1]{|{#1}|}
%% \newcommand{\isDefined}{=_{def}}
\newcommand{\isDefined}{\triangleq}

\newcommand{\lt}{$<$}
\newcommand{\gt}{$>$}

%% tminus: "thin minus", with less space around it;
%% telem: "thin element"
\newcommand{\tminus}{\!\! - \!\!}
\newcommand{\telem}{\! \in \!}

%% stexttt: "small" texttt
\newcommand{\stexttt}[1]{{\small \texttt{#1}}}

\newcommand{\mathify}[1]{\mathord{\mbox{#1}}}
\newcommand{\italMathId}[1]{\mathify{\textit{\textrm{#1}}}}
\newcommand{\romanMathId}[1]{\mathify{\textup{\textrm{#1}}}}
\newcommand{\ttMathId}[1]{\mathify{\textup{\texttt{#1}}}}

\newcommand{\ttsub}[2]{${\ttMathId{#1}}_{#2}$}
\newcommand{\ttsup}[2]{${\ttMathId{#1}}^{#2}$}
\newcommand{\mttsub}[2]{{\ttMathId{#1}}_{#2}}
\newcommand{\twoarray[2]}{\begin{array}{l}  #1 \\ #2 \end{array}}


% \newcommand{\CBS}{\begin{leftbar}}
% \newcommand{\CBE}{\end{leftbar}}
\newcommand{\CBS}{}
\newcommand{\CBE}{}


%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}

%\newenvironment{proof}[1][Proof]{\begin{trivlist}\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{definition}[1][Definition]{\begin{trivlist}\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{example}[1][Example]{\begin{trivlist}\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{remark}[1][Remark]{\begin{trivlist}\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

%\newcommand{\qed}{\nobreak \ifvmode \relax \else
%      \ifdim\lastskip<1.5em \hskip-\lastskip
%      \hskip1.5em plus0em minus0.5em \fi \nobreak
%      \vrule height0.75em width0.5em depth0.25em\fi}


==> greater_figure.tex <==
\begin{figure*}[t]
\centering
\begin{minipage}{0.24\textwidth}
\centering
\begin{minted}[fontsize=\small, frame=single,framesep=2pt,escapeinside=||]{java}
... 
if( |\setlength{\fboxrule}{1pt}\cfbox{lightblueborder}{\textbf{x > 1}}| ) { 
  ... 
} 
...
\end{minted}
\end{minipage}
\hspace{10mm}
\begin{minipage}{0.48\textwidth}
\centering
\includegraphics[height=5cm,keepaspectratio]{figures/greater_fig.png}
%\caption{}
\end{minipage}
\label{fig:greater}
\caption{The expression \scode{x > 1} is generated given its surrounding code context. At each step, the model generates the next node in $path_1$ and $path_2$ using the root path $\mathcal{R}$. Dashed lines denote AST parent-child relations; solid lines denote AST paths.}
\end{figure*}

==> packages.tex <==
%!TEX root=draft.tex
\usepackage[dvipsnames,usenames]{color}
\usepackage{fancyvrb}
\usepackage{setspace}
\usepackage{url}
\usepackage[dvipsnames]{xcolor}
\usepackage{paralist}
\usepackage[small,compact]{titlesec}
\usepackage{setspace}
\usepackage{times}
\usepackage{paralist}
\usepackage{amsmath,amssymb,amsfonts,amsthm}
\usepackage[geometry,clock]{ifsym}
\usepackage[T1]{fontenc}
\usepackage[latin9]{inputenc}
\usepackage[dvipsnames,usenames]{color}
\usepackage{listings}
\usepackage{float}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{pifont}% http://ctan.org/pkg/pifont
\usepackage{epsfig}
% A good source for fonts:
% http://tex.stackexchange.com/questions/213835/using-many-typewriter-fonts-in-a-single-document
\usepackage{txfonts}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{rotating}
\usepackage{mathpartir}
\usepackage{array}
\usepackage{todonotes}
\usepackage[percent]{overpic}
\usepackage{ragged2e}
\usepackage{fancybox}
%\usepackage{pstricks}
\usepackage{hyperref}
\usepackage[nolist,nohyperlinks]{acronym}
\usepackage{multirow}
\usepackage{tikz}
\usepackage{xspace} % makes sure we have spaces before next word, but not before punctuation.
\usepackage{lastpage}
%\usepackage{slashbox}
\usepackage{enumitem}
%\usepackage{enumerate}

\usepackage{mathtools} 

\usepackage{booktabs}


\usepackage{framed}




==> remove_java_examples.tex <==
\begin{figure}[t]
\centering
%\begin{tabular}[t]{c}
\noindent\rule{\textwidth}{1pt}
\begin{subfigure}[t!]{1.02\textwidth}
\vspace{2mm}
\begin{minted}[fontsize=\footnotesize, frame=single,framesep=2pt,escapeinside=||]{Java}
public void updatePipeline(
    String clientName, ExtendedBlock oldBlock, ExtendedBlock newBlock, 
    DatanodeID[] newNodes, String[] storageIDs) throws IOException {
  UpdatePipelineRequestProto req = UpdatePipelineRequestProto.newBuilder()
    .setClientName(clientName).setOldBlock(PBHelper.convert(oldBlock))
    .setNewBlock(PBHelper.convert(newBlock))
    .addAllNewNodes(Arrays.asList(PBHelper.convert(newNodes)))
    .addAllStorageIDs(
      storageIDs == null ? null : |\greenbox{Arrays.asList(storageIDs)}|) 
    .build();
  try {
    rpcProxy.updatePipeline(null, req);
  } catch (ServiceException e) {
    throw ProtobufHelper.getRemoteException(e);
  }
}
\end{minted}
\end{subfigure}
\\
\vspace{1mm}

\begin{subfigure}[]{0.9\textwidth}
\footnotesize
\centering
\begin{tabular}{|l|lr|}
\hline
\bf{Model}  & \bf{Predictions} &  \\
\Xhline{4\arrayrulewidth}
True ref:                            & \texttt{Arrays.asList(storageIDs)} & \\
\Xhline{4\arrayrulewidth}
\multirow{3}{*}{TLM (this work)}             & \texttt{storageIDs[0]} & (13.9\%) \\
                                 & \textbf{\texttt{Arrays.asList(storageIDs)}} & (3.6\%) \\
                                 & \texttt{storageIDs.convertTo(storageIDs)} & (2.6\%) \\
\Xhline{4\arrayrulewidth}
\multirow{3}{*}{Transformer-base +copy}             & \texttt{storageIDs.convert(newBlocks)} & \\
                                 & \texttt{storageIDs.convert(newNodes)} & \\
                                 & \texttt{storageIDs.clone()} &\\
\hline
\multirow{3}{*}{BiLSTM$\rightarrow$LSTM +copy}     & \texttt{stoargeIDs.toCase()} & \\
                                 & \texttt{storageIDs.clone()}  & \\
                                 & \texttt{storageIDs.getBytes()} & \\
\hline
\multirow{3}{*}{Seq2tree +copy}             & \texttt{storageIDs.convert(newNodes)} & \\
                                 & \texttt{storageIDs.convert(newBlock)}  & \\
                                 & \texttt{storageIDs.convert(storageIDs)} & \\
\hline
\end{tabular}
\vspace{2mm}
\end{subfigure} \\
\noindent\rule{\textwidth}{1pt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\vspace{2mm}
%\noindent\rule{\textwidth}{1pt}

\begin{subfigure}[t!]{1.0\textwidth}
\vspace{2mm}
\begin{minted}[fontsize=\footnotesize, frame=single,framesep=2pt,escapeinside=||]{Java}
public void refreshLoadedJobCache() {
  if (getServiceState() == STATE.STARTED) {
    if (storage instanceof CachedHistoryStorage) {
      ((CachedHistoryStorage) storage).refreshLoadedJobCache();
    } else {
      throw new UnsupportedOperationException(
        storage.getClass().getName() 
        + " is expected to be an instance of " 
        + |\greenbox{CachedHistoryStorage.class.getName()}|);
    }
  } else {
    LOG.warn("Failed to execute refreshLoadedJobCache: 
      ... JobHistory service is not started");
  }
}
\end{minted}
\end{subfigure}
\\
\vspace{1mm}

\begin{subfigure}[]{0.9\textwidth}
\footnotesize
\centering
\begin{tabular}{|l|lr|}
\hline
\bf{Model}  & \bf{Prediction} &  \\
\Xhline{4\arrayrulewidth}
True ref:                            & \texttt{} & \\
\Xhline{4\arrayrulewidth}
\multirow{3}{*}{TLM (this work)}             & \texttt{\textbf{CachedHistoryStorage.class.getName()}} & (56.9\%) \\
                                 & \texttt{e.getClass().getName()} & (3.0\%) \\
                                 & \texttt{applicationNamesInfo.getClass().getName()} & (1.5\%) \\
\Xhline{4\arrayrulewidth}
\multirow{3}{*}{Transformer-base +copy}             & \texttt{storage.getClass().getName()} & \\
                                 & \texttt{getClass().getName()} & \\
                                 & \texttt{getServiceState()} &\\
\hline
\multirow{3}{*}{BiLSTM$\rightarrow$LSTM +copy}     & \texttt{getClass().getName()} & \\
                                 & \texttt{getClass().getSimpleName()}  & \\
                                 & \texttt{this.getClass().getName()} & \\
\hline
\multirow{3}{*}{Seq2tree +copy}             & \texttt{storage.getClass()} & \\
                                 & \texttt{getClass().getName()}  & \\
                                 & \texttt{storage.getName()} & \\
\hline
\end{tabular}
\vspace{2mm}
\end{subfigure} \\\vspace{2mm}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Second Java Page %%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]
\begin{subfigure}[t!]{1.01\textwidth}
\vspace{2mm}
\begin{minted}[fontsize=\footnotesize, frame=single,framesep=2pt,escapeinside=||]{Java}
public synchronized String moveApplication(ApplicationId appId, 
    String queueName) throws YarnException {
  SchedulerApplication<FSAppAttempt> app = applications.get(appId);
  if (app == null) {
    throw new YarnException("App to be moved " + appId + " not found.");
  }
  FSAppAttempt attempt = (FSAppAttempt) app.getCurrentAppAttempt();
  synchronized (attempt) {
    FSLeafQueue oldQueue = (FSLeafQueue)|\greenbox{app.getQueue()}|;
    FSLeafQueue targetQueue = queueMgr.getLeafQueue(queueName, false);
    if (targetQueue == null) {
      throw new YarnException("Target queue " + queueName 
        + " not found or is not a leaf queue.");
    }
    if (targetQueue == oldQueue) {
      return oldQueue.getQueueName();
    }
    if (oldQueue.getRunnableAppSchedulables().contains(attempt)) {
      verifyMoveDoesNotViolateConstraints(attempt, oldQueue, targetQueue);
    }
    executeMove(app, attempt, oldQueue, targetQueue);
    return targetQueue.getQueueName();
  }
}
\end{minted}
\end{subfigure}
\\
\vspace{1mm}

\begin{subfigure}[]{0.9\textwidth}
\footnotesize
\centering
\begin{tabular}{|l|lr|}
\hline
\bf{Model}  & \bf{Prediction} &  \\
\Xhline{4\arrayrulewidth}
True ref:                            & \texttt{app.getQueue()} & \\
\Xhline{4\arrayrulewidth}
\multirow{3}{*}{TLM (this work)}             & \texttt{attempt.getQueue()} & (15.7\%) \\
                                 & \texttt{\textbf{app.getQueue()}} & (11.6\%) \\
                                 & \texttt{attempt.get(queueName)} & (9.2\%) \\
\Xhline{4\arrayrulewidth}
\multirow{3}{*}{Transformer-base +copy}             & \texttt{attempt.getQueue()} & \\
                                 & \texttt{\textbf{app.getQueue()}} & \\
                                 & \texttt{attempt.getLeafQueue()} &\\
\hline
\multirow{3}{*}{BiLSTM$\rightarrow$LSTM +copy}     & \texttt{attempt.clone()} & \\
                                 & \texttt{attempt.getLeafQueue()}  & \\
                                 & \texttt{attempt.getObject()} & \\
\hline
\multirow{3}{*}{Seq2tree +copy}             & \texttt{attempt.getQueue()} & \\
                                 & \texttt{\textbf{app.getQueue()}}  & \\
                                 & \texttt{app.getMetaData()} & \\
\hline
\end{tabular}
\vspace{2mm}
\end{subfigure} \\\vspace{2mm}
\noindent\rule{\textwidth}{1pt}
\begin{subfigure}[t!]{1.0\textwidth}
%\vspace{2mm}
\begin{minted}[fontsize=\footnotesize, frame=single,framesep=2pt,escapeinside=||]{Java}
public List<NodeReport> getNodeReports(NodeState... states) 
    throws YarnException, IOException {
  EnumSet<NodeState> statesSet = (states.length == 0) ? 
      |\greenbox{EnumSet.allOf(NodeState.class)}| : EnumSet.noneOf(NodeState.class);
  for (NodeState state : states) {
    statesSet.add(state);
  }
  GetClusterNodesRequest request = 
    GetClusterNodesRequest.newInstance(statesSet);
  GetClusterNodesResponse response = rmClient.getClusterNodes(request);
  return response.getNodeReports();
}
\end{minted}
\end{subfigure}
\\
\vspace{1mm}

\begin{subfigure}[]{0.9\textwidth}
\footnotesize
\centering
\begin{tabular}{|l|lr|}
\hline
\bf{Model}  & \bf{Prediction} &  \\
\Xhline{4\arrayrulewidth}
True ref:                            & \texttt{EnumSet.allOf(NodeState.class)} & \\
\Xhline{4\arrayrulewidth}
\multirow{3}{*}{TLM (this work)}             & \texttt{\textbf{EnumSet.allOf(NodeState.class)}} & (32.6\%) \\
                                 & \texttt{EnumSet.empty} & (10.2\%) \\
                                 & \texttt{new LinkedHashSet()} & (3.1\%) \\
\Xhline{4\arrayrulewidth}
\multirow{3}{*}{Transformer-base +copy}             & \texttt{Collections.emptyList()} & \\
                                 & \texttt{Arrays.asList(states)} & \\
                                 & \texttt{Collections.<NodeState> emptyList()} & (\emph{Syntax error})\\
\hline
\multirow{3}{*}{BiLSTM$\rightarrow$LSTM +copy}     & \texttt{ImmutableSet.of()} & \\
                                 & \texttt{ImmutableList.of()}  & \\
                                 & \texttt{EnumSet.noneOf(NodeState.class)} & \\
\hline
\end{tabular}
\end{subfigure} \\\vspace{2mm}

\caption{Java examples from our test set along with the predictions of our model and the baselines.}
\label{appendix_java_figure}
\end{figure} 


\begin{subfigure}[t!]{1.01\textwidth}
\vspace{2mm}
\begin{minted}[fontsize=\scriptsize, frame=single,framesep=2pt,escapeinside=||]{Java}
public void setup(Context context) throws IOException, InterruptedException {
  conf = context.getConfiguration();
  syncFolders = conf.getBoolean(DistCpOptionSwitch.SYNC_FOLDERS.getConfigLabel(), false);
  ignoreFailures = conf.getBoolean(DistCpOptionSwitch.IGNORE_FAILURES.getConfigLabel(), false);
  skipCrc = conf.getBoolean(|\greenbox{DistCpOptionSwitch.SKIP\_CRC}|.getConfigLabel(), false);
  overWrite = conf.getBoolean(DistCpOptionSwitch.OVERWRITE.getConfigLabel(), false);
  append = conf.getBoolean(DistCpOptionSwitch.APPEND.getConfigLabel(), false);
  preserve = DistCpUtils.unpackAttributes(
               conf.get(DistCpOptionSwitch.PRESERVE_STATUS.getConfigLabel()));
  targetWorkPath = new Path(conf.get(DistCpConstants.CONF_LABEL_TARGET_WORK_PATH));
  Path targetFinalPath = new Path(conf.get(DistCpConstants.CONF_LABEL_TARGET_FINAL_PATH));
  targetFS = targetFinalPath.getFileSystem(conf);
  if (targetFS.exists(targetFinalPath) && targetFS.isFile(targetFinalPath)) {
    overWrite = true;
  }
  if (conf.get(DistCpConstants.CONF_LABEL_SSL_CONF) != null) {
    initializeSSLConf(context);
  }
}
\end{minted}
\end{subfigure}
\\
\vspace{1mm}

\begin{subfigure}[]{0.9\textwidth}
\footnotesize
\centering
\begin{tabular}{|l|lr|}
\hline
\bf{Model}  & \bf{Prediction} &  \\
\Xhline{4\arrayrulewidth}
True ref:                            & \texttt{DistCpOptionSwitch.SKIP\_CRC} & \\
\Xhline{4\arrayrulewidth}
\multirow{3}{*}{TLM (this work)}             & \texttt{\textbf{DistCpOptionSwitch.SKIP\_CRC}} & (91.5\%) \\
                                 & \texttt{DistCpOptionSwitch.CRC} & (1.3\%) \\
                                 & \texttt{DistCpOptionSwitch.SKIP\_CRC.get(0)} & (0.4\%) \\
\Xhline{4\arrayrulewidth}
\multirow{3}{*}{Transformer-base +copy}             & \texttt{DistCpOptionSwitch.SYNC\_FOLDERS} & \\
                                 & \texttt{DistCpOptionSwitch.SYNC\_FOLDERS.getConfigLabel()} & \\
                                 & \texttt{DistCpOptionSwitch.OVERWRITE} &\\
\hline
\multirow{3}{*}{BiLSTM$\rightarrow$LSTM +copy}     & \texttt{DistCpOptionSwitch.CRC.getConfigLabel()} & \\
                                 & \texttt{DistCpOptionSwitch.OVERWRITE.getConfigLabel()}  & \\
                                 & \texttt{DistCpOptionSwitch.SKIP\_FAILURES.getConfigLabel()} & \\
\hline
\multirow{3}{*}{Seq2tree +copy}             & \texttt{DistCpOptionSwitch.OVERWRITE\_FAILURES.getConfigLabel()} & \\
                                 & \texttt{DistCpOptionSwitch.IGNORE\_FAILURES.getConfigLabel()}  & \\
                                 & \texttt{DistCpOptionSwitch.OVERWRITE.getConfigLabel()} & \\
\hline
\end{tabular}
\end{subfigure} \\\vspace{2mm}

\begin{subfigure}[t!]{1.0\textwidth}
\vspace{2mm}
\begin{minted}[fontsize=\footnotesize, frame=single,framesep=2pt,escapeinside=||]{Java}
static int getSplitRatio(int nMaps, int nRecords, Configuration conf) {
  int maxChunksIdeal = getMaxChunksIdeal(conf);
  int minRecordsPerChunk = getMinRecordsPerChunk(conf);
  int splitRatio = getSplitRatio(conf);
  if (nMaps == 1) {
    LOG.warn("nMaps == 1. Why use DynamicInputFormat?");
    return 1;
  }
  if (nMaps > maxChunksIdeal)
    return splitRatio;
  int nPickups = (int) Math.ceil((float) maxChunksIdeal / nMaps);
  int nRecordsPerChunk = (int) Math.ceil(
      |\greenbox{(float) nRecords}| / (nMaps * nPickups));
  return nRecordsPerChunk < minRecordsPerChunk ? splitRatio : nPickups;
}
\end{minted}
\end{subfigure}
\\
\vspace{1mm}

\begin{subfigure}[]{0.9\textwidth}
\footnotesize
\centering
\begin{tabular}{|l|lr|}
\hline
\bf{Model}  & \bf{Prediction} &  \\
\Xhline{4\arrayrulewidth}
True ref:                            & \texttt{(float) nRecords} & \\
\Xhline{4\arrayrulewidth}
\multirow{3}{*}{TLM (this work)}             & \texttt{\textbf{(float) nRecords}} & (12.9\%) \\
                                 & \texttt{(float) conf} & (5.7\%) \\
                                 & \texttt{(float) nMaps} & (3.5\%) \\
\Xhline{4\arrayrulewidth}
\multirow{3}{*}{Transformer-base +copy}             & \texttt{\textbf{(float) nRecords}} & \\
                                 & \texttt{(nRecords * nRecords)} & \\
                                 & \texttt{(nMaps * nRecords)} &\\
\hline
\multirow{3}{*}{BiLSTM$\rightarrow$LSTM +copy}     & \texttt{(nPickups * nPickups)} & \\
                                 & \texttt{(nPickups * nMaps)}  & \\
                                 & \texttt{(nPickups * nRecords)} & \\
\hline
\multirow{3}{*}{Seq2tree +copy}             & \texttt{(double) nPickups} & \\
                                 & \texttt{(maps nPickups nPickups)}  & (\emph{Syntax error}) \\
                                 & \texttt{(nPickups - nPickups)} & \\
\hline
\end{tabular}
\vspace{2mm}
\end{subfigure} \\\vspace{2mm}


==> specificmacros.tex <==
%!TEX root=draft.tex

\newcommand{\EY}[2]{ {\color{red} #1 (\textbf{EY}: \emph{#2})} }
% \newcommand{\YD}[2]{ {\color{ForestGreen} #1 (\textbf{YD}: \emph{#2})} }
% \newcommand{\NP}[2]{ {\color{purple} #1 (\textbf{NP}: \emph{#2})} }

\newcommand{\tool}{\scode{GitZ}\xspace}

\newcommand{\demonsmarker}{\textbf{DEMONS START HERE, IF NOT EARLIER}}

\newcommand{\neighbrel}{\tilde{\delta}}
\newcommand{\neighb}[2]{\neighbrel(#1,#2)}

% programming languages
\newcommand{\Python}{\scode{Python}\xspace}
\newcommand{\CSharp}{\scode{C\#}\xspace}

% other
\newcommand{\Github}{\scode{Github}\xspace}

% text formatting
\newcommand{\sectionette}[1]{\vspace{1pt}\noindent \textit{#1}:}
\newcommand{\para}[1]{\vspace{3pt}\noindent\textbf{\textit{#1}}}
\newcommand{\scode}[1]{{\small \texttt{#1}}}
\newcommand{\tcode}[1]{{\scriptsize \texttt{#1}}}
\newcommand{\sname}[1]{{\small \textsc{#1}}}

% colors
\definecolor{airforceblue}{rgb}{0.36, 0.54, 0.66}
\definecolor{awesome}{rgb}{1.0, 0.13, 0.32}
\definecolor{blue(pigment)}{rgb}{0.2, 0.2, 0.6}
\definecolor{britishracinggreen}{rgb}{0.0, 0.26, 0.15}
\definecolor{cadmiumgreen}{rgb}{0.0, 0.42, 0.24}
\definecolor{carminered}{rgb}{1.0, 0.0, 0.22}
\definecolor{electricindigo}{rgb}{0.44, 0.0, 1.0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\hypersetup{colorlinks=true,linkcolor=black, citecolor=black, urlcolor=black}

\definecolor{javared}{rgb}{0.6,0,0} % for strings
\definecolor{javagreen}{rgb}{0.25,0.5,0.35} % comments
\definecolor{javapurple}{rgb}{0.5,0,0.35} % keywords
\definecolor{javadocblue}{rgb}{0.25,0.35,0.75} % javadoc

%\definecolor{path-red}{HTML}{B85450}
%\definecolor{path-blue}{HTML}{6C8EBF}
\definecolor{path-orange}{HTML}{D79B00}
\definecolor{path-green}{HTML}{517040}

\usepackage{listings}
\lstset{language=Java,
    basicstyle=\ttfamily,
    keywordstyle=\color{javapurple}\bfseries,
    stringstyle=\color{javared},
    commentstyle=\color{javagreen},
    morecomment=[s][\color{javadocblue}]{/**}{*/},
    %numbers=left,
    numberstyle=\tiny\color{black},
    stepnumber=2,
    numbersep=10pt,
    tabsize=4,
    showspaces=false,
    showstringspaces=false,
    showlines=true
}

\newcommand{\rulesep}{\unskip\ \vrule\ }

% lstlistings styles
%\lstset{basicstyle=\ttfamily\scriptsize,
%        language=C,
%        emph={},
%        emphstyle={\underbar},
%        numbers=none,
%        numberfirstline=false,
%        numberstyle=\tiny\color{mygray},
%        escapeinside={(*@}{@*)}}

%\newcommand{\f1}{0.58}
\newcommand{\fscore}{$0.58$}



==> task_example_fig.tex <==
\newcommand{\specialcell}[2][l]{%
  \begin{tabular}[#1]{@{}l@{}}#2\end{tabular}}
\begin{figure*}[t]
%\centering
\begin{minipage}{0.65\textwidth}
\begin{minted}[fontsize=\scriptsize, frame=single,framesep=2pt,escapeinside=||]{java}
Path getPath(int curId, int limitPerDir, Type type) {
  if (curId <= 0) { return basePath; }
  String name = "";
  switch(type) {
    case FILE:
      name = FILE_PREFIX + 
        new Integer(curId % limitPerDir).toString(); break;
    case DIRECTORY:
      name = DIR_PREFIX + 
        new Integer(curId % limitPerDir).toString(); break;
  }
  Path base = getPath((curId / limitPerDir), 
    limitPerDir, Type.DIRECTORY);
  return  |\setlength{\fboxrule}{1pt}\cfbox{green}{new Path(base, name)}|;
}
\end{minted}
\end{minipage}
%\begin{minipage}{0.48\textwidth}
\begin{minipage}{0.34\textwidth}
\begin{subfigure}[t]{1\textwidth}
\scriptsize
\raggedright
\small{Generated: (Java)}
\begin{tabular}{lr}
\scode{\scriptsize new Path(base, name)} & (19.3\%) \\
\scode{\scriptsize new Path(base)} & (10.6\%) \\
\scode{\scriptsize new Path(name, base)} & (10.0\%) 
\end{tabular}
\caption{}
\label{fig:task_example_a}
\end{subfigure}
\end{minipage}
\begin{minipage}{0.5\textwidth}
\begin{minted}[fontsize=\scriptsize, frame=single,framesep=2pt,escapeinside=||]{csharp}
int TrailingSpaces(this StringBuilder builder)                                                                                                               
{                                
  var bound = builder.Length - 1;                                                                                                                                        
  if (builder.Length == 0) return 0;                                                                                                                                     
  if (builder[bound] != ' ') return 0;                                                                                                                                   
  var c = 0;                                                                                                                                                             
  for (var i = bound; i <= bound; i--)                                                                                                                                   
  {                                                                                                                                                                      
    if (i < 0) break;                                                                                                                                                  
    if (|\setlength{\fboxrule}{1pt}\cfbox{green}{builder[i]}| != ' ') break;                                                                                                                                      
    c++;                                                                                                                                                               
  }                                                                                                                                                                      
  return c;                                                                                                                                                              
} 
\end{minted}
\end{minipage}
\begin{minipage}{0.37\textwidth}
\begin{subfigure}[t]{1\textwidth}
\scriptsize
\raggedright
\small{Generated: (C\#)}
\begin{tabular}{lr}
\scode{\scriptsize builder[i]} & (62.2\%) \\
\scode{\scriptsize c[i]} & (2.6\%) \\
\scode{\scriptsize builder.length} & (1.8\%) 
%\scode{\scriptsize universeFunc(optionUniverse)} & (8.7\%) \\
%\scode{\scriptsize optionUniverse(optionUniverse)} & (5.9\%) \\
%\specialcell[b]{\scode{\scriptsize optionUniverse as} \\ \;\;\;\;\;\;\;\;\scode{\scriptsize OptionFilterUniverse}} & (3.6\%) 
\end{tabular}
\caption{}
\label{fig:task_example_b}
\end{subfigure}
\end{minipage}
\caption{\aeg{} examples from our test sets, along with the predicted expressions by our model.}
\label{fig:task_example}
\end{figure*}

